X-ray Absorption and Reflection in Active Galactic Nuclei

X-ray spectroscopy offers an opportunity to study the complex mixture of emitting and absorbing components in the circumnuclear regions of active galactic nuclei, and to learn about the accretion process that fuels AGN and the feedback of material to their host galaxies. We describe the spectral signatures that may be studied and review the X-ray spectra and spectral variability of active galaxies, concentrating on progress from recent Chandra, XMM-Newton and Suzaku data for local type 1 AGN. We describe the evidence for absorption covering a wide range of column densities, ionization and dynamics, and discuss the growing evidence for partial-covering absorption from data at energies > 10 keV. Such absorption can also explain the observed X-ray spectral curvature and variability in AGN at lower energies and is likely an important factor in shaping the observed properties of this class of source. Consideration of self-consistent models for local AGN indicates that X-ray spectra likely comprise a combination of absorption and reflection effects from material originating within a few light days of the black hole as well as on larger scales. It is likely that AGN X-ray spectra may be strongly affected by the presence of disk-wind outflows that are expected in systems with high accretion rates, and we describe models that attempt to predict the effects of radiative transfer through such winds, and discuss the prospects for new data to test and address these ideas.

==> table.tex <==
% For tables use
\begin{table}
% table caption is above the table
\caption{Black Hole Mass, 2-10 keV Fluix and Orbital Timescale at 10$r_g$}
\label{tab:1}       % Give a unique label
% For LaTeX tables use
\begin{tabular}{lccc}
\hline\noalign{\smallskip}
Target & BH Mass & 2-10 keV Flux & T$_{\rm orb}$ \\
 & /$10^6 {\rm M}_{\odot}$ & /$10^{-11}\, {\rm erg\, s^{-1}\, cm^{-2}}$ & ks \\
\noalign{\smallskip}\hline\noalign{\smallskip}
IC 4329A$^a$ & 1 & 7.0 & 1.01 \\
MCG-6-30-15$^b$ & 2 & 4.0 & 2.02 \\
NGC 4051 $^a$ & 2 & 2.0 * 2.02 \\
NGC 5506$^c$ & 2 &  7.0 & 2.02 \\
Mrk 766$^d$ & 4 & 2.0 & 4.05 \\
Mrk 335$^e$ & 5 & 1.0 & 5.06 \\
NGC 7314$^f$ & 5 & 4.0 & 5.06 \\
NGC 7469$^e$ & 7 & 3.2 & 7.08 \\
NGC 4593$^e$ & 8 & 4.5 & 8.10 \\
NGC 4151$^a$ & 13 & 10.0 & 13.16
MCG+8-11-11$^g$ & 15 & 2.3 & 15.18 \\
NGC 3516$^e$ & 23 & 5.0 & 23.27 \\
NGC 3783$^a$ & 29 & 7.0 & 29.35 \\
NGC 3227$^e$ & 44 & 2.8 & 44.52 \\
NGC 2992$^e$ & 52 & 0.4 & 52.62 \\
MCG--5-23-16$^g$ & 70 & 9.0 & 70.84 \\
Mrk 509$^e$ & 72 & 6.6 & 72.86 \\
Fairall 9$^e$ & 81 & 2.5 & 81.97 \\
MR 2251-178$^h$ & 98 & 5.0 & 99.17 \\
NGC 7213$^e$ & 98 & 3.0 & 99.17 \\
Mrk 841$^e$ & 100 & 1.0 & 101.19 \\
NGC 5548$^e$ & 110 & 5.0 & 111.31 \\
Arp 102B$^i$ & 140 & 1.1 & 141.67 \\
NGC 2110$^e$ & 200 & 3.5 & 202.39 \\
MCG--2-58-22$^g$ & 350 & 3.3 & 354.18 \\ 



\end{tabular}
\end{table}


